Completeness of Logical Atomicity for Linearizability in Concurrent Separation Logic

Linearizability is a standard correctness condition for concurrent data structures. It guarantees that operations behave as if they took effect at some atomic instant between their call and return points. Despite the central role linearizability plays, prior work has argued for instead using a style of specification that internalizes the atomicity of operations in terms of the logic's reasoning rules, known as logical atomicity. These logically atomic specifications are intended to be easier to compose inside of the logic than linearizability. Prior work has shown that in the Iris separation logic framework, a certain form of logically atomic specifications implies that a data structure is linearizable. However, the converse remained an open question: for every linearizable data structure, is it always possible to derive a corresponding logically atomic specification? This paper resolves this question in the affirmative. We prove a completeness theorem for Iris that derives a logically atomic specification for any linearizable data structure. As a consequence, we are able to embed a variety of linearizability proof techniques into Iris and use them to derive logically atomic specifications. We apply this to three linearizability proof methods: aspect-oriented linearizability proofs, forward simulations with commit points, and meta-configuration tracking. Using these embeddings, we derive logically atomic specifications for the Herlihy-Wing queue and the Baskets Queue. We furthermore establish a connection between logical atomicity and an encoding of refinement in Iris that has been used in prior logical relations models. This result allows us to transport logically atomic specifications across refinements, which we apply to the Folly MPMC queue implementation. All of the results in this paper have been mechanized in the Rocq Prover.

==> body/keyideas.tex <==
\section{Key Ideas}

%


==> body/logatom.tex <==
\section{Logical Atomicity via Linearizability}\label{sec:logatom}

Although linearizability is a standard correctness condition for concurrent data structures, in many concurrent separation logics it is common to instead use an alternate form of specification based on \emph{logical atomicity}.
Whereas linearizability captures atomicity by relating traces to sequential specifications, logical atomicity instead characterizes atomicity in terms of what logical reasoning rules an atomic operation should support.
In particular, by asking what special reasoning rules the logic provides for primitive physically atomic operations, and then proving similar rules for the operations of a concurrent data structure, we allow clients of the data structure to reason \emph{as if} these operations were physically atomic.
And, what is special about physically atomic operations in many CSLs are the rules for interacting with \emph{invariant assertions}.
Thus, logically atomic specifications establish similar rules for working with invariants.

In particular, in Iris, the invariant assertions have the form $\knowInv{}{R}$ which says that assertion $R$ is an invariant, meaning that it holds before and after each step of execution.
Unlike regular assertions in a separation logic, the assertion $\knowInv{}{R}$ is \emph{persistent}, meaning that it can be duplicated and shared by multiple threads, \ie $\knowInv{}{R}\proves\knowInv{}{R}\ast\knowInv{}{R}$.
Atomicity is captured by the following invariant access rule.\footnote{The full version of this rule annotates invariant assertions with a \emph{namespace} identifier, which is used to prevent opening the same invariant twice. These matters are orthogonal concerns and we omit these annotations here.}
$$\inferhref{InvAccPhysical}{rule:inv-acc}
{\proves\{P\ast \later R\}\,e\,\{\Ret v. Q\ast \later  R\}\\\atomic(e)}
{\knowInv{}{R}\proves \{P\}\,e\,\{\Ret v. Q\}}$$
To prove a specification under an invariant $\knowInv{}{R}$, the rule says that we can open this invariant and add $R$ to the precondition, as long as we reestablish $R$ in the postcondition.
The side condition $\atomic(e)$ means $e$ is physically atomic, \ie in the operational semantics, $e$ reduces to a value in a single execution step.
Because $e$ reduces to a value in a single step, this rule preserves the property that the invariant $R$ must hold before and after each step.
The later modality ``$\later$'' guarding $R$ is needed to make nesting of impredicative invariants sound.
For so-called \emph{timeless} assertions that do not involve impredicative nesting, this later modality can be removed.
Although our proof uses an impredicative invariant, we only need to access its impredicative part after the program has taken one step, so this later modality is not a problem for our proof and we will ignore it afterwards.

For a logically atomic operation, the idea is to similarly allow for an invariant to be opened around the atomic point at which the operation takes effect.
Following a style pioneered by the TaDA~\citep{da-rocha-pinto2014-tada} logic, Iris supports such specifications through an alternate version of the Hoare triple called a \emph{logically atomic triple}, $\ahoare{P}{e}{\Ret v.Q}$.
The most important rules are shown below.%
\footnote{Like the \heaplang{} logic, the actual rules about the logically atomic triple in Iris are also stated in terms of $\wprename$.}
\begin{mathpar}
\inferhref{InvAccLogical}{rule:inv-acc-logatom}
{\proves\ahoare{P\ast \later R}{e}{\Ret v. Q\ast \later R}}
{\knowInv{}{R}\proves \ahoare{P}{e}{\Ret v. Q}}
\and
\inferhref{LaIntro}{rule:logatom-intro}
{\proves \All \Phi. \hoare{\AU_{P,Q}(\Phi)}{e}{\Phi}}{\proves\ahoare{P}{e}{\Ret v. Q}}
\and
\inferhref{AuFire}{rule:au-fire}
{\proves\hoare{P}{e_a}{Q}\\\atomic(e_a)}{\proves\hoare{\AU_{P,Q}(\Phi)}{e_a}{\Phi}}
\end{mathpar}
Crucially, the logically atomic triple also provides an invariant access rule \ruleref{rule:inv-acc-logatom}, but notice here that $e$ is \emph{not} necessarily physically atomic.
To initially prove a logically atomic triple about a data structure's operations, we use \ruleref{rule:logatom-intro} to reduce it to a Hoare triple with an \emph{atomic update} assertion $\AU$ as precondition and an arbitrary postcondition $\Phi$.
Because $\Phi$ is universally quantified, the only way for the data structure to obtain the postcondition $\Phi$ is to use \ruleref{rule:au-fire} to ``fire'' the $\AU_{P,Q}(\Phi)$.
The point at which this rule is applied corresponds to the linearization point of the operation.
At the linearization point, the data structure first obtains $P$ from the $\AU$, and it must then prove $Q$ immediately after executing one physical step.

The goal of this paper is to relate such logically atomic specifications to linearizability.
In particular, we will show that the following combination of (\ref{eq:init-spec}) a Hoare triple about an object's initialization, and (\ref{eq:op-spec}) a logically atomic triple about the object's operations, is equivalent to linearizability:
\begin{align}
  &\mathleftalign{\atomspec[\mu]{\IsP}{\PState}{\function{init}}{\function{op}}\eqdef} \notag \\
  &\hspace*{4em} \vdash \hoare{\TRUE}{\function{init}()}{\Ret \textit{obj}. \Exists \gamma.\IsP(\gamma,\textit{obj})\ast\PState(\gamma,s_0)} \label{eq:init-spec}\\
  &\hspace*{4em} \pure{\textit{vr}(x)} \ast \IsP(\gamma,\textit{obj})\vdash\ahoare{\PState(\gamma,s)}{\function{op}(\textit{obj},x)}{\Ret y.\Exists s'.\PState(\gamma,s')\ast\pure{\textit{rr}(s,x,s',y)}} \label{eq:op-spec}\\
  &\hspace*{4em}  \All \gamma, \textit{obj} . \persistent{\IsP(\gname,\textit{obj})}
\end{align}
This specification is parameterized by $\mu$, \ie a sequential specification for the object, and two predicates, $\IsP$ and $\PState$.
The $\IsP$ assertion is a persistent assertion that states that an object is a valid instance of this class of objects, \eg satisfies some internal invariant of the data structure; $\PState$ describes the current abstract state of the object.
These assertions are connected by a \emph{ghost name} $\gamma$, which ensures both assertions talk about the same object.
The specification for $\function{init}$ returns ownership of both of these assertions about the newly created object.
Then, the specification for $\function{op}$ requires that the request and the object must both be valid, and that $\function{op}$ atomically updates the object from state $s$ to state $s'$ and returns $y$ in accord with the $\textit{rr}$ relation.

\citet{birkedal2021-free} prove that such a specification implies linearizability.
\begin{theorem}[Logical Atomicity $\Ra$ Linearizability \cite{birkedal2021-free}]\label{thm:logatom-soundness}
$$\atomspec[\mu]{\IsP}{\PState}{\function{init}}{\function{op}}\implies\lin[\mu]{\function{init}}{\function{op}}$$
\end{theorem}

We call this result a soundness theorem for logical atomicity because it connects the logical notion to the external linearizability property.\footnote{This theorem is a consequence of a more general result which we
discuss further in \Cref{sec:free-theorem}.}
In this paper, we prove a result that is essentially the converse of this soundness theorem, \ie a completeness theorem for logical atomicity.
The direct converse looks as follows.
\begin{proposition}\label{prop:logatom}
  $\lin[\mu]{\function{init}}{\function{op}}\implies\Exists\IsP,\PState. \atomspec[\mu]{\IsP}{\PState}{\function{init}}{\function{op}}$
\end{proposition}
As we will see, our proof strategy requires modifying this statement slightly, for reasons we explain next.

\subsection{Proof Strategy}
The difficult part of the proof is in deriving the logically atomic triple about $\function{op}$.
To do so, we apply \ruleref{rule:logatom-intro}, which reduces the goal to deriving a Hoare triple about the function.
Because of the assumption that the data structure is linearizable, we know that the $\function{op}$ function is safe.
That is, it never gets stuck.
Thus, we can use the proof rules of Iris to reason step by step as the operation executes.
However, at some point we must fire the atomic update introduced by \ruleref{rule:logatom-intro}.
This point must correspond to what is essentially a linearization point of the operation.
Since, by assumption, the data structure is linearizable, given a trace of call and return operations, this linearizability assumption will tell us where we can insert such linearization points, and therefore fire the atomic update.
To use this assumption, we create an Iris invariant that stores an annotated trace of all of the call and return operations that have been executed so far.
When we reach a point that is a linearization point in the annotated trace, we know that we can therefore fire the atomic update.
However, there are two complications to this basic idea that pose challenges:
\begin{enumerate}
\item[C\textsubscript{1}] \textbf{Future-dependent linearization points}.
While proving a logically atomic triple, one only knows the historic trace $\vv*{t}{h}$ up to the current point of execution.
From this partial historic trace, we can obtain a linearized trace $\vv*{t}{h}'$ that adds the linearization point annotations to $\vv*th$.
Suppose we fire atomic updates as we go according to this extension $\vv*{t}{h}'$.
After a new call or return event $u$, the trace will be extended by $u$ to become $\phytr = \vv*{t}{h}\dplus u$.
By linearizability, we can obtain another linearization $\anntr$ of the new trace.
Although $\phytr$ is obtained by appending a new event to $\vv*{t}{h}$, the definition of linearizability \emph{does not} guarantee that $\anntr$ can also be obtained by adding some new events to $\vv*{t}{h}'$.
In fact, $\anntr$ can choose completely different linearization points from $\vv*{t}{h}'$.
This phenomenon is well-known as future-dependent linearization, and was observed in the very first work that proposed linearizability~\cite{herlihy1990-linearizability}.
The problem is that if $\anntr$ uses different linearization points than $\vv*{t}{h}'$, we would have to amend the $\AU$\uq s we have already fired, which is not possible.
\item[C\textsubscript{2}] \textbf{External linearization points}.
Proving a logically atomic triple requires firing the $\AU$ at a specific program step, \ie one must find a particular physically atomic operation to fire the $\AU$, while the linearization points extracted from applying the definition of linearizability are just some $\textlog{Lin}$ events in an annotated trace.
The definition of linearizability does not tell us specific physical steps tied to these $\textlog{Lin}$ events.
This means that to use the linearization points extracted from $\trlinname$, we must find a way to map these events to some physical steps.
\end{enumerate}

Challenge 1 is solved by using \emph{prophecy variables}~\cite{jung2019-proph,adadi1991-hpv,DBLP:conf/tamc/ZhangFFSL12}.
Prophecy variables allow for ``predicting'' what the outcomes of future program steps will be during the course of a proof.
Using prophecy variables, one can prophesy the complete
trace of operations on an object at the time the object is created.
Thus, we can extract all linearization points once and for all from this complete trace, and do not have to worry about the linearization points shifting when extending partial traces with new events.

Challenge 2 is solved by a technique called \emph{helping}~\cite{spies2022-later,herlihy1991-wait-free,	DBLP:conf/podc/Censor-HillelPT15}.
Rather than trying to fire the atomic update for an operation at a specific physical step, we instead store $\AU$ assertions for all operations that are in the middle of execution in a shared invariant.
When an operation is called and emits a $\textlog{Call}$ event, we add its $\AU$ to the invariant.
Linearization itself happens at the $\textlog{Call}$ and $\textlog{Ret}$ events of operations: whenever an operation emits a $\textlog{Call}$ or $\textlog{Ret}$ event, we gather the $\AU$ assertions for all pending operations whose $\textlog{Lin}$ events occur in the annotated trace just prior to this event, extract them from the invariant, and fire all of them.
We then store the corresponding $\Phi$ assertions resulting from each back inside the invariant, so that they can later be collected by the corresponding operation.
This means one physical step, \ie the step on which an operation emits its $\textlog{Call}$ or $\textlog{Ret}$ event, can linearize multiple operations, not limited to the $\AU$ of the operation taking the step.
Thus, an operation logically ``helps'' others perform their $\AU$.

Readers familiar with carrying out proofs of logical atomicity in Iris will not be surprised that we end up using prophecy variables and helping in our proof.
Indeed, these techniques are familiar and often used in proving the logical atomicity of specific data structures.
This pattern of transferring atomic updates for helping has been used from the very beginning in Iris logical atomicity proofs, and prophecy variables were specifically added to Iris in order to reason about future-dependent linearizability.
What makes our results novel is the generality we work at, and the fact that we show that these two techniques suffice to do \emph{all} such logical atomicity proofs.



\subsection{Data Structure Wrapper}\label{sec:logatom-wrapper}
\begin{figure}
\begin{minipage}{0.3\linewidth}
\begin{align*}
&\textit{wrapi}(\function{init})()\eqdef\\
&\quad(\function{init}(),\ghostcode{\NewProph})
\end{align*}
\end{minipage}%
\begin{minipage}{0.7\linewidth}
\begin{align*}
&\textit{wrapo}(\function{op})(\textit{objp},x)\eqdef\\
&\quad\Let (\textit{obj},\ghostcode{p}) := \textit{objp} in\\
&\quad\Let \ghostcode{\tau} := \ghostcode{\NewGhostID} in \ghostcode{\Resolve p to \Inl (\tau,x)};\\
&\quad\Let y := \function{op}(\textit{obj},x) in \ghostcode{\Resolve p to \Inr (\tau,y)}; y
\end{align*}
\end{minipage}
\caption{Wrapped Data Structure Methods}\label{fig:wrapper}
\end{figure}

In order to use prophecy variables to ``predict'' the future stream of call and return operations, we need to annotate the operations with a wrapper that attaches the prophecy variables to the events we want to predict.
In Iris, prophecy variables are implemented by two special ``virtual'' operations: $\ghostcode{\langkw{newproph}}$ and $\ghostcode{\langkw{resolve}}$.
These operations are virtual in the sense that the behavior of the program will not change after erasing them.
The specifications for working with these primitives are as follows.
\begin{mathpar}
\inferhref{ProphNe}{rule:proph-ne}
{}{\proph{\prophid_1}{\vv*v1}\ast\proph{\prophid_2}{\vv*v2}\proves\pure{\prophid_1\neq\prophid_2}}
\and
\inferhref{HtNewProph}{rule:wp-newproph}
{}{\hoare{\TRUE}{\ghostcode{\NewProph}}{\Ret \prophid.\Exists \vv\val.\proph{\prophid}{\vv\val}}}
\and
\inferhref{HtResolve}{rule:wp-resolve}
{}{\hoare{\proph{\prophid}{\vv\val}}{\ghostcode{\Resolve \prophid to \valB}}{\Ret \TT.\Exists \vv\val'.\pure{\vv\val=\valB::\vv\val'}\ast\proph{\prophid}{\vv\val'}}}
\end{mathpar}
Operation $\ghostcode{\NewProph}$ allocates a fresh prophecy variable $\prophid$.
Resource $\proph{\prophid}{\vv\val}$ in its postcondition says that the resolutions on $\prophid$ in the future execution of the program will be the values in the list $\vv\val$.
It is an exclusive resource ensuring the thread currently owning $\proph{\prophid}{\vv\val}$ is the only thread allowed to resolve $\prophid$.
Under precondition $\proph{\prophid}{\vv\val}$, primitive $\ghostcode{\Resolve \prophid to \valB}$ \emph{resolves} prophecy variable $\prophid$ to value $\valB$.
The resolution guarantees that the first element in $\vv\val$ must be $\valB$, and removes this element from the future resolutions list.

Using these operations, we define wrappers for data structures as shown in \Cref{fig:wrapper}.
The wrapped $\function{init}$ function associates a prophecy variable with the newly created object.
The wrapped $\function{op}$ function allocates a fresh tag for this invocation of the operation using a helper function $\ghostcode{\NewGhostID}$, and resolves the associated prophecy variable before $\function{op}$ is called and after $\function{op}$ returns.
These two resolutions capture the call and return events of the invocation, where the event $(\tau,\textlog{Call}(x))$ is encoded as $\Inl(\tau,x)$, and event $(\tau,\textlog{Ret}(y))$ is encoded as $\Inr(\tau,y)$.

To generate the fresh tag with $\ghostcode{\NewGhostID}$, we can in fact reuse the prophecy variable mechanism, by treating the prophecy variable's identifier as the tag. Since $\proph{\prophid}{\vv\val}$ is exclusive, we can discard the $\vv\val$ part and just use the prophecy variable $\prophid$ itself as a unique ghost token.
Thus, we define $\ghostcode{\NewGhostID}$ as follows, and derive the following helper specifications:
\begin{mathpar}
\ghostcode{\NewGhostID}\eqdef\ghostcode{\NewProph}
\and
\ghostToken{\tau}\eqdef\Exists\vv\val.\proph{\tau}{\vv\val}
\and
\inferhref{HtNewGhostID}{rule:wp-newghostid}
{}{\hoare{\TRUE}{\ghostcode{\NewGhostID}}{\Ret \tau.\ghostToken{\tau}}}
\and
\inferhref{TokenNe}{rule:token-ne}
{}{\ghostToken{\tau_1}\ast\ghostToken{\tau_2}\proves \pure{\tau_1\neq\tau_2}}
\end{mathpar}

Because we resolve the call and return events using the prophecy variable, this means that when we first create the prophecy variable during the wrapped initialization, the list of values $\vv\val$ in the $\proph{\prophid}{\vv\val}$ permission will be the entire trace of events on the data structure.
Thus, we can define a derived predicate, $\prophtrace[\textit{obj}]{\rho}{\prophid}{\phytr}$ that asserts ownership of the prophecy variable $\prophid$ and says that starting from configuration $\rho$, the decoded list of prophesied values is a call/return trace $\phytr$ generated by a valid interaction between the data structure and a client, \ie $\Exists \rho'.\rho\advsteps{\phytr}\rho'$.
Predicate $\textlog{prophTrace}$ is encoded using a technique inspired by typed prophecy variables~\cite{jung2019-proph}.%
\footnote{The encoding requires the use of the law of excluded middle because proposition $\Exists \rho'.\rho\mathrel{\smash{\advsteps{\phytr}}}\rho'$ is generally undecidable~\cite{rice1953}.}
The full definition of $\textlog{prophTrace}$ is included in \Cref{sec:app:typed-proph}.


\subsection{Invariant}\label{sec:logatom-inv}



\begin{figure}
\begin{align*}
&\Exists \gamma_\pi,\gamma_e,\gamma_\phi,\gamma_s,\vv\pi,\vv e,\pstate,\Phi s,s,\anntr.\textlog{let}\,\conf:=(\vv\pi,\vv e,\pstate)\,\textlog{in}\quad\ownGhost{\gamma}{\Square(\gamma_\pi,\gamma_e,\gamma_\phi,\gamma_s)}\\
&\ast\ownGhost{\gamma_\pi}{\authfull \textit{l2m}(\textit{activeOp}(\vv\pi))}
\ast\ownGhost{\gamma_e}{\authfull\vv{\expr}}
\ast\ownstate(\pstate)
\ast\ownGhost{\gamma_s}{\authfull \mapsingleton{0}{s}}
\ast\prophtrace[\textit{obj}]{\conf}{p}{\pi_\Sigma(\anntr)}\tag{P\textsubscript{1}}\label{fig:I-atom-part-own}\\
&\ast\ownGhost{\gamma_\phi}{\authfull \Phi s}\ast\left(\Sep_{\tau\gets \Phi\in\Phi s} \textit{interpret}(\anntr,\tau,\Phi)\right)
\tag{P\textsubscript{2}}\label{fig:I-atom-part-au}\\
&\ast\left(\Sep_{\tau\in\vv{\pi}.1}\ghostToken{\tau}\right)\tag{P\textsubscript{3}}\label{fig:I-atom-part-token}\\
&\ast\pure{\textit{pendingOp}(\anntr)\subseteq\dom(\Phi s)=\{\vv{\pi}.1\}}\tag{P\textsubscript{4}}\label{fig:I-atom-part-dom}\\
&\ast\pure{\textlog{partial-well-formed}_{\textlog{lin}}(\anntr)
\land(\Exists s'.\textlog{sound}_\mu(\pi_{\textlog{lin}}(\anntr),s,s'))
\land\cfgsafe{\vv\pi}{\vv e}{\pstate}}\tag{P\textsubscript{5}}\label{fig:I-atom-part-lin}
\end{align*} %
$$\text{where }\textit{interpret}(\anntr,\tau,\Phi)\eqdef\begin{array}[t]{@{}l@{ }l}
\multicolumn{2}{@{}l}{\textlog{match}\,\pi_\tau(\anntr)\,\textlog{with}}\\
\mid(\_,\textlog{Call}(\_))::\_&\Ra\FALSE\\
\mid(\_,\textlog{Lin}(x,\_))::\_&\Ra\AU_{\PState_\mu(\gamma,s),\Ret y.\Exists s'.\PState_\mu(\gamma,s')\ast\pure{\textit{rr}(s,x,s',y)}}(\Phi)\\
\mid(\_,\textlog{Ret}(y))::\_&\Ra\Phi(y)\\
\mid\nil&\Ra\TRUE\\
\textlog{end}&
\end{array}$$


\caption{The Definition of $I_{\textlog{atom}_\mu}(\gamma,\textit{obj},p)$}\label{fig:I-atom-def}
\end{figure}
As mentioned above, the proof needs an invariant that relates the abstract state of the object to the physical state, and tracks the correspondence between the trace prophecy and what atomic updates have been completed.
Specifically, for an object $\textit{obj}$ associated with the ghost resource name $\gamma$,
we use an invariant $\knowInv{}{I_{\textlog{atom}_\mu}(\gamma,\textit{obj},p)}$.
Here $p$ is the prophecy variable used to speculate the future trace of $\textit{obj}$.

At a high level, the invariant relates four things: the current configuration $\conf=(\vv\pi,\vv e,\pstate)$ of the object and pending operations, the abstract sequential specification state $s$ of $\textit{obj}$, a store $\Phi s$ of the atomic updates and receipts of the operations currently in flight, and a prophecy $\anntr$ of the object's future trace.
The future trace predicts where each pending operation will linearize so that the invariant can tell for every in-flight operation whether it has already linearized or not.
We use this information to track the status of each operation's atomic update.

$\knowInv{}{I_{\textlog{atom}_\mu}(\gamma,\textit{obj},p)}$ is defined in \Cref{fig:I-atom-def}.
It consists of five parts: \ref{fig:I-atom-part-own} tracks the system status, \ref{fig:I-atom-part-au} stores the atomic updates and receipts, \ref{fig:I-atom-part-token} and \ref{fig:I-atom-part-dom} enforce its internal consistency, and \ref{fig:I-atom-part-lin} ensures that the remaining future trace is linearizable.
We now describe each of these pieces in more detail.

\paragraph{\ref{fig:I-atom-part-own}: System Status}
Along with the physical points-tos and the prophecy trace, the status of the object is tracked by several pieces of ghost state that are combined together on this line of the invariant to track components of the object.

\begin{itemize}
\item The current configuration $\conf=(\vv \pi,\vv\expr,\pstate)$. It is tracked by three pieces of resources:
    \begin{itemize}
    \item Authoritative resource $\ownGhost{\gamma_\pi}{\authfull\textit{l2m}(\textit{activeOp}(\vv\pi))}$ tracks pending operations, \ie the operations that have been called but not yet returned.
    Here, function $\textit{activeOp}$ returns operations that are not $\bot$, and function $\textit{l2m}$ converts an association list $(A\times B)^*$ to a finite map $A\fpfn B$.
    The fragmentary copy of this state is kept in the proof environment.
    \item Authoritative resource $\ownGhost{\gamma_e}{\authfull\vv{\expr}}$ tracks other threads spawned by operations. %
    \item $\ownstate(\pstate)$ asserts the ownership of the data structure's physical state, defined as $\Sep_{(\ell\gets\val)\in\pstate}\ell\mapsto\val$, \ie the ownership of each location in $\pstate$.
    \end{itemize}

\item The abstract sequential state $s$ of the object: $\ownGhost{\gamma_s}{\authfull \mapsingleton{0}{s}}$.\footnote{The actual Iris mechanization does not use ghost map but another type of ghost state known as exclusive authoritative state.}

\item The prophecy to the future trace $\anntr$: $\prophtrace[\textit{obj}]{\conf}{p}{\pi_\Sigma(\anntr)}$.
\end{itemize}

\paragraph{\ref{fig:I-atom-part-au}: Atomic Updates and Receipts}
Recall that $\AU(\Phi)$ provides a receipt $\Phi$ after being fired, and this receipt is specified by a client of the data structure.
An operation learns the type of the receipt when it is called.
Because of helping, the current operation can be linearized by another operation.
To make this work, we need a mapping between operations and their receipt types so that the helper and helpee agree on what the receipt is.
This is represented by the authoritative ghost resource $\ownGhost{\gamma_\phi}{\authfull \Phi s}$ for the receipt map $\Phi s$.
Note that this is a higher-order ghost state because $\Phi s$ contains Iris propositions.
Alongside this map, this part of the invariant stores, for each pending operation with tag $\tau$, either its atomic update or its receipt, selected by the function $\textit{interpret}$ according to the next event of $\tau$ in the future trace $\anntr$.
An operation $\tau$ in $\Phi s$ thus has four possible stages:
\begin{enumerate}
\item The next event of $\tau$ is $\textlog{Call}(x)$, meaning that $\tau$ has not been called yet. This case is impossible because uncalled operations are not pending, and thus should not be in $\Phi s$.
\item The next event of $\tau$ is $\textlog{Lin}(x,y)$, meaning that $\tau$ has been called, but has yet to linearize.
In this case, the invariant stores an atomic update for this operation.
The pre- and postconditions of the $\AU$ come from specification (\ref{eq:op-spec}), and the type of the receipt comes from $\Phi s$.
\item The next event of $\tau$ is $\textlog{Ret}(y)$, meaning that $\tau$ has linearized, but has not returned yet.
In this case, the invariant stores the receipt of this operation.
\item Tag $\tau$ is not in $\anntr$, meaning that $\tau$ has returned.
In this case, the mission of the invariant for this operation is done, and the invariant stores nothing about the operation.
\end{enumerate}

\paragraph{\ref{fig:I-atom-part-token}: Ghost Tokens}
This part is an iterated separating conjunction of ghost tokens for all tags in $\vv{\pi}.1$ for two purposes.
First, the exclusiveness of ghost tokens ensures that there is no duplication of tags in $\vv\pi$.
Second, because the tag of a new operation is generated by $\ghostcode{\NewGhostID}$, tokens are used to prove the freshness of a new tag.

\paragraph{\ref{fig:I-atom-part-dom}: Consistency of the Status}
The pending operation list $\vv\pi$, the receipt map $\Phi s$, and the future trace $\anntr$ all talk about pending operations, so this part ensures they describe the same set: the domain of $\Phi s$ coincides with the tags appearing in $\vv\pi$, and the pending operations $\textit{pendingOp}(\anntr)$ extracted from the future trace are among them.
The subset inclusion $\textit{pendingOp}(\anntr)\subseteq\dom(\Phi s)$ is not necessarily an equality because $\textit{pendingOp}$ is a conservative under-approximation: under partial correctness an operation may be called and never return, in which case its tag is indistinguishable from one that has already returned.
The precise definition of $\textit{pendingOp}$ and the lemmas relating it to trace extension are given in \Cref{sec:app:invariant-consistency}.

\paragraph{\ref{fig:I-atom-part-lin}: Partial Linearizability of Future Trace}
This part ensures the future trace $\anntr$ is a suffix of a linearizable trace.
First, for each tag, the call, linearization, and return events of it must occur in order, but unlike $\textlog{well-formed}_{\textlog{lin}}$, the first event does not have to be $\textlog{Call}$.
$$\textlog{partial-well-formed}_{\textlog{lin}}(\anntr)\eqdef\All \tau.\Exists v,v'.\pi_\tau(\anntr)\substrof[(\tau,\textlog{Call}(v));(\tau,\textlog{Lin}(v,v'));(\tau,\textlog{Ret}(v'))]$$
Here, $\vv x\substrof\vv y$ means $\vv x$ is a subtrace of $\vv y$, \ie $\vv x$ can be obtained by taking consecutive elements from $\vv y$.
Second, the linearization events in the future coincide with the sequential behavior $\mu$.
Third, the current configuration is safe, \ie its pending operations and other threads will never get stuck under the most adversarial interaction.
$$\cfgsafename(\rho)\eqdef \All \phytr, \vv\pi\!',\vv\expr\!',\pstate'.\rho\advsteps{\phytr}(\vv\pi\!',\vv\expr\!',\pstate')\Ra\All {e\in\vv\pi\!'.2\dplus\vv\expr\!'}.e\in\Val\lor\red(e,\pstate')$$
Properties of $\textlog{partial-well-formed}_{\textlog{lin}}$ and $\cfgsafename$ used in the proof are collected in \Cref{sec:app:invariant-partial-lin}.

\paragraph{Additional Auxiliary Resources}
The invariant also carries an agreement ghost resource $\ownGhost{\gamma}{\Square(\gamma_\pi,\gamma_e,\gamma_\phi,\gamma_s)}$ to link four ghost names used by $I_{\textlog{atom}}$ to the single ghost name $\gamma$ exposed by $\IsP$.
The agreement ghost resource is a persistent assertion such that ${\ownGhost{\gamma}{\Square x}\ast\ownGhost{\gamma}{\Square y}\proves\pure{x=y}}$.


\paragraph{The Construction of\/ $\IsP$ and\/ $\PState$}
The validity of an object and the assertion for its abstract state are defined on top of $I_{\textlog{atom}_\mu}$.
\begin{align*}
\IsP_\mu(\gamma,v)&\eqdef \Exists \textit{obj}, \prophid. \pure{v=(\textit{obj},\prophid)}\ast \knowInv{}{I_{\textlog{atom}_\mu}(\gamma,\textit{obj},\prophid)}\\
\PState_\mu(\gamma,s)&\eqdef\Exists\gamma_\pi,\gamma_e,\gamma_\phi,\gamma_s.\ownGhost{\gamma}{\Square(\gamma_\pi,\gamma_e,\gamma_\phi,\gamma_s)}\ast0\hookrightarrow^{\gamma_s}s
\end{align*}
$\IsP_\mu$ is a thin wrapper around $I_{\textlog{atom}_\mu}$ and
$\PState_\mu$ is the ownership of the fragmentary part of the abstract state.
The agreement resource ensures $\gamma_s$ is the same ghost name used in $I_{\textlog{atom}_\mu}$.
Although $\PState_\mu$ is independent of the sequential behavior $\mu$, we still add the $\mu$ subscript to emphasize that it is a specific construction used to prove a logically atomic triple about $\mu$.



\subsection{Proof Sketch}\label{sec:logatom-proof}
Since we need the prophecy variable to make this proof work, we can only prove the logical atomicity of the wrapped version of the data structure.
Thus, we restate \Cref{prop:logatom} as below:
\begin{theorem}[Linearizability $\Ra$ Logical Atomicity]\label{thm:logatom}
$$\lin[\mu]{\function{init}}{\function{op}}\land\nofork{\function{init}()}{\varnothing}\implies\atomspec[\mu]{\IsP_\mu}{\PState_\mu}{\textit{wrapi}(\function{init})}{\textit{wrapo}(\function{op})}$$
where
$\nofork{\expr}{\pstate}\eqdef\All \vv\expr\!',\pstate'.([\expr],\pstate)\tpsteps(\vv\expr\!',\pstate')\Ra|\vv\expr\!'|=1$
\end{theorem}

Due to a technical restriction, we can only prove the theorem when the $\function{init}$ function is sequential, as specified by $\nofork{\function{init}()}{\varnothing}$.
This is typically not a problem in practice because a concurrent data structure rarely spawns internal helping threads.

We sketch the proof here; a more detailed walk-through is given in \Cref{sec:app:logatom-proof}.
We must show that the wrapped operations satisfy the logically atomic specification, reasoning under the invariant $I_{\textlog{atom}_\mu}$ of \Cref{fig:I-atom-def}.
After initialization, the argument follows the life cycle of an operation invocation.

\paragraph{Initialization}
Running $\textit{wrapi}(\function{init})$ creates the object with initial state $\ownstate(\pstate)$ and allocates its prophecy variable $\prophtrace{(\nil,\nil,\pstate)}{p}{\phytr}$.
Because the data structure is linearizable, the prophesied trace $\phytr$ is guaranteed to be the physical projection of some linearizable annotated trace $\anntr$.
This is exactly what is needed to establish $I_{\textlog{atom}_\mu}$ for the empty initial configuration.
After creating the associated ghost state and invariant, we return the assertions $\IsP_\mu$ and $\PState_\mu$ in the postcondition.

\paragraph{Operation Invocation}
The prophesied future trace records, for every pending operation, where its linearization point will be.
When the wrapped operation resolves its call event, we open the invariant and consult this prophecy: every operation whose linearization point in the prophecy falls before this call is helped.
For each helped operation, we fire its stored atomic update, advance the object's abstract state through the corresponding sequential transition, and replace the fired update with the receipt it produces.
The current operation is then registered, with its own atomic update stored for later.

The internal steps of $\function{op}$ merely preserve the invariant.
For each internal step, since it is safe (by assumption of linearizability), we use the stored physical state in the invariant to justify the step, and then update the configuration and state in the invariant.
The proof of this part follows the same pattern as Theorem 17 of \citet{hostert2026-completeness}.

Finally, resolving the \emph{return} event performs any remaining helping and extracts this operation's receipt, which is precisely the postcondition demanded by its logically atomic triple.





